Improving the Thresholds of Generalized LDPC Codes with Convolutional Code Constraints

CC-GLPDC codes are a class of generalized low-density parity-check (GLDPC) codes where the constraint nodes (CNs) represent convolutional codes. This allows for efficient decoding in the trellis with the forward-backward algorithm, and the strength of the component codes easily can be controlled by the encoder memory without changing the graph structure. In this letter, we extend the class of CC-GLDPC codes by introducing different types of irregularity at the CNs and investigating their effect on the BP and MAP decoding thresholds for the binary erasure channel (BEC). For the considered class of codes, an exhaustive grid search is performed to find the BP-optimized and MAP-optimized ensembles and compare their thresholds with the regular ensemble of the same design rate. The results show that irregularity can significantly improve the BP thresholds, whereas the thresholds of the MAP-optimized ensembles are only slightly different from the regular ensembles. Simulation results for the AWGN channel are presented as well and compared to the corresponding thresholds.

==> tikz.tex <==





\begin{figure}[t]
	\centering
	\subfigure[Rate $1/2$ trellis (left) in a constraint node (right).]
	{ \scalebox{0.9}{
	        \begin{tikzpicture}[scale=.7]
            \tikzstyle{varnode}=[circle,thick,draw=black!100,fill=black!100,minimum size=1mm]
            \tikzstyle{checknode}=[rectangle,thick,draw=black!100,fill=black!100,minimum size=4mm]
            \tikzstyle{statenode}=[circle,thick,draw=black,double,fill=black!0,minimum size=1mm]
            \tikzstyle{constnode}=[rectangle,line width=.4mm,draw=black!100,fill=black!0,minimum size=7mm]
            \tikzstyle{varcsnode}=[rectangle,thick,draw=black!0,fill=black!0,minimum size=.001]
            % define nodes first
            
            \node (vu1) at (1,1) [varnode,label=above:$v_{p,1}^{(1)}$] {};
            \node (c1) at  (1,0) [checknode] {};
            \node (vl1) at (1,-1) [varnode,label=below:$u_1^{(1)}$] {};
            \node (vs1) at (0,0) [statenode] {};
           
            \draw [-] (vu1) to (c1);
            \draw [-] (vl1) to (c1);
            \draw [-] (vs1) to (c1); 
    
            \node (vu2) at (2+1,1) [varnode,label=above:$v_{p,2}^{(1)}$] {};
            \node (c2) at  (2+1,0) [checknode] {};
            \node (vl2) at (2+1,-1) [varnode,label=below:$u_2^{(1)}$] {};
            \node (vs2) at (2+0,0) [statenode] {};
           
            \draw [-] (vs2) to (c1);
            \draw [-] (vu2) to (c2);
            \draw [-] (vl2) to (c2);
            \draw [-] (vs2) to (c2); 
            \node (vs3) at (2+2,0) [statenode] {};
            \draw [-] (vs3) to (c2); 
            
            
            \node (vs4) at (5,0) [statenode] {};
            \draw [dotted] (vs3) -- (vs4);
            \node (vu4) at (6,1) [varnode,label=above:$v_{p,(d_c-1)N}^{(1)}$] {};
            \node (c4) at  (6,0) [checknode] {};
            \node (vl4) at (6,-1) [varnode,label=below:$u_{(d_c-1)N}^{(1)}$] {};
            \draw [-] (vs4) to (c4);
            \draw [-] (vu4) to (c4);
            \draw [-] (vl4) to (c4);
            \node (vs5) at (7,0) [statenode] {};
            \draw [-] (c4) to (vs5);
     
     
            % constraint node at the right side
            \node (cs1) at (10,1.25) [constnode,label=above:$$] {$N$};
            \node (vcs1) at (8.5,-1) [varcsnode,label=above:$$] {};
            \node (vcs2) at (10.5,-1) [varcsnode,label=above:$$] {};
            \node (vcs3) at (12,-1) [varcsnode,label=above:$$] {};
            
            % just for the labels
            \node (vcs11) at (8.5,-1.8)  [varcsnode,label=above:$\boldsymbol{u}^{(1)}$] {};
            \node (vcs21) at (11,-1.8) [varcsnode,label=above:$\boldsymbol{u}^{(d_c-1)}$] {};
            \node (vcs31) at (12.2,-1.8) [varcsnode,label=above:$\boldsymbol{v}_{p}$] {};
            
            \draw [-] (vcs1) to (cs1);
            \draw [-] (vcs2) to (cs1);
            \draw [-] (vcs3) to (cs1);
            
            \draw [dotted] (9.3,-1.3) to (9.55,-1.3);            
            
            \end{tikzpicture}
    % 		\label{fig:r12trellis}
    	}}
	\hfill
	\subfigure[Trellis section at time $t$ after puncturing to rate $(d_c-1)/d_c$.]
	{\scalebox{0.9}{
    \begin{tikzpicture}[scale=.9]
    \tikzstyle{varnode}=[circle,thick,draw=black,fill=black!100,minimum size=1.5mm]
    \tikzstyle{pvarnode}=[circle,thick,draw=black,fill=black!0,minimum size=1.5mm]
    \tikzstyle{checknode}=[rectangle,thick,draw=black!100,fill=black!100,minimum size=4mm]
    \tikzstyle{statenode}=[circle,thick,draw=black,double,fill=black!0,minimum size=3mm]
            % define nodes first
            
            \node (vu1) at (1,1) [varnode,label=above:${v}_{p,t}$] {};
            \node (c1) at  (1,0) [checknode] {};
            \node (vl1) at (1,-1) [varnode,label=below:${u}_t^{(1)}$] {};
            \node (vs1) at (0,0) [statenode] {};
           
            \draw [-] (vu1) to (c1);
            \draw [-] (vl1) to (c1);
            \draw [-] (vs1) to (c1); 
    
            \node (vu2) at (2+1,1) [pvarnode,label=above:$$] {};
            \node (c2) at  (2+1,0) [checknode] {};
            \node (vl2) at (2+1,-1) [varnode,label=below:${u}_t^{(2)}$] {};
            \node (vs2) at (2+0,0) [statenode] {};
           
            \draw [-] (vs2) to (c1);
            \draw [-] (vu2) to (c2);
            \draw [-] (vl2) to (c2);
            \draw [-] (vs2) to (c2); 
            \node (vs3) at (2+2,0) [statenode] {};
            \draw [-] (vs3) to (c2); 
         
            \node (vs4) at (5,0) [statenode] {};
            \draw [dotted] (vs3) to (vs4);
            
            \node (vu3) at (2+1+1+2,1) [pvarnode,label=above:$$] {};
            \node (c3) at  (2+1+1+2,0) [checknode] {};
            \node (vl3) at (2+1+1+2,-1) [varnode,label=below:${u}_t^{(d_c-1)}$] {};
            \node (vs5) at (5+2,0) [statenode] {};
            
            \draw [-] (vs5) to (c3);
            \draw [-] (vs4) to (c3);
            \draw [-] (vu3) to (c3);
            \draw [-] (vl3) to (c3);
            
    \end{tikzpicture}
	}}
	\\
		\caption{Factor graph representation of a constraint node trellis.}\label{fig:puncturedtrellis15}
		\vspace*{-2mm} 
	\label{fig:constnode15}
\end{figure}

==> tikz/ccgldpc_rate12.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5.53in,
height=4.712in,
at={(0.928in,0.636in)},
scale only axis,
xmin=0,
xmax=1.5,
xlabel style={font=\color{white!15!black}},
xlabel={$E_b/N_0$ (dB)},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BER},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.154,0.932)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.0pt, mark size=4.3pt, mark=diamond*, mark options={solid, fill=red, red}]
  table[row sep=crcr]{%
-1	0.17060546875\\
-0.5	0.150048828125\\
0	0.124560546875\\
0.25	0.099306640625\\
0.5	0.069931640625\\
0.625	0.05626953125\\
0.75	0.019892578125\\
0.875	0.00337158203125\\
1	1.93359375e-06\\
1.1	1.77734375e-06\\
1.2	1.318359375e-06\\
1.3	1.42578125e-06\\
};
\addlegendentry{Optimized BP(ir), $N=102400$}

\addplot [color=blue, dashdotted, line width=1.0pt, mark size=1.8pt, mark=square*, mark options={solid, fill=blue, blue}]
  table[row sep=crcr]{%
-1	0.17857421875\\
-0.5	0.163037109375\\
0	0.142744140625\\
0.25	0.12849609375\\
0.5	0.116025390625\\
0.75	0.105849609375\\
1	0.090751953125\\
1.1	0.08072265625\\
1.15	0.0101018415178571\\
1.205	0.000158476360103627\\
1.21	5.16467524509804e-05\\
1.215	2.02523895307289e-05\\
};
\addlegendentry{Optimized MAP(ir), $N=102400$}

\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
0.6761	1e-08\\
0.6761	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized BP(ir)}

\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
1.0616	1e-08\\
1.0616	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized MAP(ir)}

\end{axis}

\begin{axis}[%
width=7.135in,
height=5.781in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> tikz/ccgldpc_rate13.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5.53in,
height=4.703in,
at={(0.928in,0.635in)},
scale only axis,
xmin=-0.5,
xmax=2,
xlabel style={font=\color{white!15!black}},
xlabel={$E_b/N_0$ (dB)},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BER},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.145,0.927)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.0pt, mark size=4.3pt, mark=diamond*, mark options={solid, fill=red, red}]
  table[row sep=crcr]{%
-1	0.199423828125\\
-0.5	0.17234375\\
0	0.04025390625\\
0.25	0.000467087765957447\\
0.5	3.47531138790036e-06\\
0.75	3.55113636363636e-06\\
0.85	3.85993083003953e-06\\
};
\addlegendentry{Optimized BP(ir), $N=102400$}

\addplot [color=blue, dashdotted, line width=1.0pt, mark=square*, mark options={solid, fill=blue, blue}]
  table[row sep=crcr]{%
-1	0.226552734375\\
-0.5	0.213818359375\\
0	0.195478515625\\
0.25	0.183427734375\\
0.5	0.1698828125\\
0.75	0.162421875\\
1	0.15013671875\\
1.25	0.127529296875\\
1.35	0.0055693359375\\
1.375	0.00350899832589286\\
1.4	0\\
1.425	0\\
};
\addlegendentry{Optimized MAP(ir), $N=102400$}

\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
-0.0046	1e-08\\
-0.0046	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized BP(ir)}

\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
1.2386	1e-08\\
1.2386	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized MAP(ir)}

\end{axis}
\end{tikzpicture}%

==> tikz/ccgldpc_rate23.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5.546in,
height=4.695in,
at={(0.93in,0.634in)},
scale only axis,
xmin=1.25,
xmax=2.75,
xlabel style={font=\color{white!15!black}},
xlabel={$E_b/N_0$ (dB)},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={BER},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.166,0.93)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.0pt, mark size=4.3pt, mark=diamond*, mark options={solid, fill=red, red}]
  table[row sep=crcr]{%
0	0.11216796875\\
0.25	0.101845703125\\
0.5	0.096259765625\\
0.75	0.08166015625\\
1	0.064638671875\\
1.25	0.053154296875\\
1.4	0.04357421875\\
1.5	0.038154296875\\
1.6	0.03318359375\\
1.8	0.0007080078125\\
2	5.68033854166667e-05\\
2.3	5.16153541226216e-06\\
2.4	3.2325802714333e-06\\
2.5	2.95060597519729e-06\\
};
\addlegendentry{Optimized BP(ir), $N=102400$}

\addplot [color=blue, dashdotted, line width=1.0pt, mark size=1.8pt, mark=square*, mark options={solid, fill=blue, blue}]
  table[row sep=crcr]{%
0	0.11474609375\\
0.25	0.1073046875\\
0.5	0.09966796875\\
0.75	0.08609375\\
1	0.074091796875\\
1.25	0.06392578125\\
1.5	0.05037109375\\
1.6	0.040908203125\\
1.7	0.00225\\
1.8	1.42240955564294e-05\\
1.85	4.57763671875e-07\\
};
\addlegendentry{Optimized MAP(ir), $N=102400$}

\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
1.6037	1e-08\\
1.6037	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized BP(ir)}

\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
1.6516	1e-08\\
1.6516	1e-06\\
};
\addlegendentry{MC-DE Thd Optimized MAP(ir)}

\end{axis}

\begin{axis}[%
width=7.156in,
height=5.76in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
